Adaptive Task Offloading for Space Missions: A State-Graph-Based Approach

Advances in space exploration have led to an explosion of tasks. Conventionally, these tasks are offloaded to ground servers for enhanced computing capability, or to adjacent low-earth-orbit satellites for reduced transmission delay. However, the overall delay is determined by both computation and transmission costs. The existing offloading schemes, while being highly-optimized for either costs, can be abysmal for the overall performance. The computation-transmission cost dilemma is yet to be solved. In this paper, we propose an adaptive offloading scheme to reduce the overall delay. The core idea is to jointly model and optimize the transmission-computation process over the entire network. Specifically, to represent the computation state migrations, we generalize graph nodes with multiple states. In this way, the joint optimization problem is transformed into a shortest path problem over the state graph. We further provide an extended Dijkstra's algorithm for efficient path finding. Simulation results show that the proposed scheme outperforms the ground and one-hop offloading schemes by up to 37.56% and 39.35% respectively on SpaceCube v2.0.

==> Sentence.tex <==
In addition to industry growing interest, academic
researchers have eagerly jumped into the development of small
satellites.

However, despite of great potential of FSO communication, its performance is limited by the adverse effects (viz., absorption, scattering, and turbulence) of the atmospheric channel. Out of these three effects, the atmospheric turbulence is a major challenge that may lead to serious degradation in the bit error rate performance of the system and make the communication link infeasible~\cite{7553489}. 

RS techniques have opened a door to helping people widen their ability to understand the earth [1], [2]. In fact, RS techniques are becoming more and more important in data-collection tasks. Information technology companies depend on RS to update their location-based services [3], [4]. Google Earth employs high-resolution (HR) RS images to provide vivid pictures of the earth s surface. Governments have also utilized RS for a variety of public services, from weather reporting to traffic monitoring [5] [7]. Nowadays, one cannot imagine a life without RS. Recent years have even witnessed a boom in RS satellites, providing for the first time an extremely large number of geographical images of nearly every corner of the earth s  surface [8]. Data warehouses of RS images are increasing daily, including images with different spectral and spatial resolutions [9], [10]. ~\cite{7486259}

==> table1.tex <==
%
\begin{tabular}{ccc} 
	%\toprule
	\rowcolor[rgb]{0.812,0.835,0.918} Product             & Processor                                                                                                                  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Computing Capability\\(GFLOPS)\end{tabular}                                     \\
	BAE RAD5545~\cite{BAERAD5545}                                           & RAD5545                                                                                                                    & 3.7                                                                                                \\
	\rowcolor[rgb]{0.914,0.922,0.961} MOOG G-Series Steppe Eagle~\cite{MOOG}                             & AMD G-Series compatible                                                                                                    & 75                                                                                                                                   \\
	Unibap iX5-100~\cite{iX5-100,bruhn2020enabling}                                        & \begin{tabular}[c]{@{}c@{}}Microchip SmartFusion2,\\AMD G-Series SOC\end{tabular}                                          & 127                                                                                                              \\
	\rowcolor[rgb]{0.914,0.922,0.961} SpaceCube v2.0~\cite{SpaceCube2.0}                                        & Xilinx Virtex 5                                                                                                            & 200                                                                                                                           \\
	SpaceCube v3.0~\cite{geist2019spacecube,SpaceCube3.0Patent}      & \begin{tabular}[c]{@{}c@{}}Xilinx Kintex UltraScale,\\ Xilinx Zynq MPSoC\end{tabular} & 590                                                                                                  \\
	\rowcolor[rgb]{0.914,0.922,0.961} MOOG V-Series Ryzen~\cite{MOOG} & AMD V-Series compatible                                                                                                    & 1000                                                                                                                                  \\
	 Xiphos Q8S~\cite{XiphosQ8S}          & Xilinx Ultrascale+                                                                                                         & 1800                                                                                                                             \\	
	\rowcolor[rgb]{0.914,0.922,0.961} Unibap iX10-100~\cite{iX10-100,bruhn2020enabling}     & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.922,0.961}}c@{}}Microchip PolarFire, \\AMD V1605b (Ryzen)\end{tabular}     & 3600                                                                                                           \\
	%\bottomrule
\end{tabular}
